Bridging the Gap between Real-world and Synthetic Images for Testing Autonomous Driving Systems

Deep Neural Networks (DNNs) for Autonomous Driving Systems (ADS) are typically trained on real-world images and tested using synthetic simulator images. This approach results in training and test datasets with dissimilar distributions, which can potentially lead to erroneously decreased test accuracy. To address this issue, the literature suggests applying domain-to-domain translators to test datasets to bring them closer to the training datasets. However, translating images used for testing may unpredictably affect the reliability, effectiveness and efficiency of the testing process. Hence, this paper investigates the following questions in the context of ADS: Could translators reduce the effectiveness of images used for ADS-DNN testing and their ability to reveal faults in ADS-DNNs? Can translators result in excessive time overhead during simulation-based testing? To address these questions, we consider three domain-to-domain translators: CycleGAN and neural style transfer, from the literature, and SAEVAE, our proposed translator. Our results for two critical ADS tasks -- lane keeping and object detection -- indicate that translators significantly narrow the gap in ADS test accuracy caused by distribution dissimilarities between training and test data, with SAEVAE outperforming the other two translators. We show that, based on the recent diversity, coverage, and fault-revealing ability metrics for testing deep-learning systems, translators do not compromise the diversity and the coverage of test data, nor do they lead to revealing fewer faults in ADS-DNNs. Further, among the translators considered, SAEVAE incurs a negligible overhead in simulation time and can be efficiently integrated into simulation-based testing. Finally, we show that translators increase the correlation between offline and simulation-based testing results, which can help reduce the cost of simulation-based testing.

==> Sections/background.tex <==
\section{Image-to-Image Translation}
\label{sec:background}
GAN-based and neural style transfer techniques represent two of the most studied image-to-image translation approaches in deep learning literature~\cite{cyclegan, pix2pix, gatys, style_review, deep_photo_style}. In this section,  we describe these approaches and discuss their limitations for the purpose of ADS testing. In the remainder of the paper, ``\emph{translator}'' indicates ``\emph{domain-to-domain translator}''.


\subsection{GAN-based Translators}
\label{subsec:cylce_gan}
GAN-based translators require two datasets as input, one from each domain, i.e., the real-world domain and the synthetic domain. Some GAN-based methods such as Pix2Pix~\cite{pix2pix} require the datasets to be paired, where each element in one set is mapped to an element in the other set. As discussed in Section~\ref{sec:intro},  pairing demands extra manual work, and heuristic methods for pairing many not be accurate. Hence, in order to enhance ADS testing, we consider CycleGAN~\cite{cyclegan} from the family of GAN-based translators that does not require dataset pairing.


CycleGAN includes four components: Two generators, denoted by $G$ and $F$,  and two discriminators, denoted by $D_X$ and $D_Y$. Let $X$ be the source dataset, and $Y$ be the target dataset. Generator $G$ maps an input $x \in X$ into an element $y$ that aligns with the distribution of  $Y$. Conversely,  generator $F$ aims to transform  elements in $Y$ to elements that belong to the distribution of $X$. Discriminator $D_X$ determines whether an input belongs to the distribution of $X$,  and  discriminator $D_Y$ performs a similar check for $Y$. To train a CycleGAN, we have to minimize two loss functions: One related to $G$ and $D_Y$, and the other related to $F$ and $D_X$. The first loss function aims to improve the generator $G$,  while keeping the information and content of the source distribution, $X$.  The second loss function improves $F$, while ensuring the content of the target distribution, $Y$. Each of the two loss functions includes three terms. The first term is used to train the discriminator related to each generator, i.e., $D_Y$ for $G$ and $D_X$ for $F$. This helps the discriminators improve and provide more accurate feedback to their respective generator. The second term is used to train the generator to deceive the discriminator. This helps the generator generate more realistic outputs in the target distribution.  The third term, known as cycle-consistency loss, operates under  the assumption that an input $x \in X$ transformed to  $\hat{y} = G(x)$ and then reverted back to $\hat{x} = F(\hat{y}) = F(G(x))$ should closely approximate $x$. This ensures that the generator $G$ keeps the high-level content of the input distribution while transforming between the two distributions. There is a dual cycle-consistency loss term for generator $F$. Note that to develop CycleGAN models,  all the four models, $F$, $G$, $D_X$ and $D_Y$ have to be trained simultaneously.

\textbf{Limitations:} CycleGAN training is unstable, a characteristic often seen in the GAN model family \cite{gan_unstable_salimans}. This instability is due to the simultaneous training of discriminator and generator models; as one improves, the other degrades. 
Specifically, improving $G$ (resp. $F$) adversely affects $D_Y$  (resp. $D_X$) and vice versa, complicating the achievement of a stable equilibrium during training. 

\iffalse

The loss function to be minimized consists of two adversarial loss terms and a cycle-consistence loss term. The adversarial loss is defined in the following for generator

\begin{align}
    \Lagr_{GAN}(G, D_Y, X, Y) = \EX\{\text{log } D_Y(y)\} + \EX\{\text{log } (1 - D_Y(G(x)))\}
\end{align}

Similar adversarial loss is defined for the generator $F$ as well.

\begin{align}
    \Lagr_{GAN}(F, D_X, X, Y) = \EX\{\text{log } D_X(x)\} + \EX\{\text{log } (1 - D_X(F(y)))\}
\end{align}

Next, a cycle-consistency loss is defined to help generators better do the domain-to-domain translation task while keeping the information and content of the source domain.

\begin{align}
    \Lagr_{cycle}(G,F) = \EX\{ ||F(G(x)) - x||_1\} + \EX\{ ||G(F(y)) - y||_1\}
\end{align}

The final loss function is the following.

\begin{align}
    \Lagr(G, F, D_X, D_Y) = & \Lagr_{GAN}(G, D_Y, X, Y) \\ &+ \Lagr_{GAN}(F, D_X, X, Y) \\ &+ \lambda \Lagr_{cycle}(G, F)
\end{align}

The generators, G and F, try to minimize this loss function while the discriminators, $D_X$ and $D_Y$ try to maximize it. 

\fi





\subsection{Neural Style Translators}
In contrast to GAN-based translators that require two datasets as input, the neural style transfer methods only require two images as input:  a \emph{style} image from the source domain, and a \emph{content} image from the target domain. Generally speaking, style is characterized by the 
specific pattern and texture of an image, while content refers to the objects in an image. Provided with a content image and a style image, neural style transfer retains the content of the content image, but adapts its style to match the style image. 


A well-known neural style method proposed by Gatys et al.~\cite{gatys} extracts style and content from the given images using  a pretrained convolutional neural network (CNN)~\cite{vgg19}. This method is grounded in the principle that the initial layers of a CNN capture low-level style information, while the deeper layers hold high-level content details.  Style is extracted from selected ``style layers" and content from ``content layers". Image style is represented by Gram matrices from each style layer, capturing feature map correlations at that level. To perform style transfer, the pretrained CNN and the style image are fixed, and only the content image is iteratively modified using a loss function with the following two terms: the \textit{style loss} and the \textit{content loss}.  The \textit{style loss} minimizes the weighted Euclidean distance between the Gram matrices of the style image and the content image to transform the style of the content image. The \textit{content loss} calculates the Euclidean distance between the feature maps of the content layers of the original content image and those of the transformed content image. This is to ensure that the content of the transformed image remains close to the original image.





\textbf{Limitations:} The style transfer method, as described above, iteratively adjusts the content image using gradient descent to minimize its loss function. This process, however, leads to a high execution time for image transformation,  rendering the approach unsuitable for online testing of ADS. 





==> Sections/discuss.tex <==
\section{Discussion}
\label{sec:discuss}



\emph{While evaluation datasets require labels, image pairing for the evaluation dataset is not necessary.}
Our objective is to develop a framework that enables realistic online testing for ADS, rather than tackling the domain-to-domain transformation or simulation-to-reality gap challenges. While for the latter challenges pairing images from the domains either for training or evaluation is common practice, image pairing for online testing is, in general, infeasible and even unnecessary. Specifically, 


In online testing, we utilize a DNN trained on real-world data and aim to conduct tests in a closed-loop environment using simulators. However, the potential discrepancies between simulated and real-world images can pose a challenge, creating barriers to trusting the results of online testing.




We note that our aim is to support a realistic online testing use case as opposed to addressing the domain transformation or the simulation to reality challenges. In online testing, we have a DNN trained on real-world data and we want to test in a closed loop environment using simulators. However, knowing that the differences between the images may lead to issues is a barrier in trusting the online testing results. 

As we have discussed, we only consider approaches that do not need pairing for training. 

Further, our assessment does not require paired datasets. 
This is in contrast to the earlier work that  has considered pairing dataset. To the best of our knowledge for lane-keeping we only have access to manually paired data that is quesitonable and also are not publicly avaiable. 

Instead of trying to pair dataset, we DID THIS. 

pairing ensures what??


The datasets might have different sizes. 



instead we show the overall distribution is getting close. 

We compare distributions and not pairing. 

\emph{Assumptions of our work.} 


\emph{SAEVAE does not lead to hallucination.}



The approach of integrating a translator into the ADS online testing is a rational and pivotal step towards enhancing the reliability and accuracy of evaluations. While this paper introduces the novel SAEVAE translator, it is essential to emphasize that we don't think of any particular translator as the only solution. Rather, the key principle we advocate is the inclusion of any translator capable of effectively bridging the gap between distinct datasets. Whether employing SAEVAE, CycleGAN, or other domain-to-domain translation techniques, the ultimate objective remains the same: to narrow the distribution disparities between real-world and simulator-generated images. Therefore, we insist that the presence of a translator within the testing cycle is indispensable, representing a critical component in ensuring the reliability and accuracy of autonomous systems under diverse and dynamic real-world conditions.

The utilization of unpaired domain-to-domain translation methods, as demonstrated by our SAEVAE approach, holds extreme significance in the context of domain adaptation for autonomous driving systems. Unlike methods that require paired datasets, such as pix2pix, unpaired techniques are inherently more adaptable to real-world scenarios where acquiring precisely matched data pairs is a formidable challenge. This is particularly salient in the domain of autonomous driving, where synthesizing a perfectly matched real-world and simulator dataset is often infeasible due to the inherent complexities and variations present on the road. By decoupling the source and target domains, unpaired methods like SAEVAE, CycleGAN, etc. enable a more flexible and practical approach to domain adaptation, ensuring that the trained ADS-DNNs are better equipped to handle the diverse and dynamic environments encountered in actual driving scenarios. 



==> Sections/old.tex <==

Neural style transfer methods process an image in two levels of \textit{style} and \textit{content}. In a general definition, style is a representation of the texture, patterns, and visual characteristics that are characteristic of a particular artwork or image.  Content refers to the objects, and recognizable elements present in an artwork or image. Neural style transfer methods try to keep the content of an input image while making its style similar to another image. One of the most well-known methods of neural style transfer is Gatys et al. \cite{??} method. In this method, we need an image, called style image, to imitate its style in the input image, called content image. To extract style and content from images, a pretrained convolutional neural network (CNN) for computer vision, such as VGG19, is used. The idea behind this method is that the first few convolutional layers of this CNN have feature maps containing low-level information about the style. The more deep layers of the CNN have feature maps conatining high-level information of the image which can be used as a representation of content. We choose several layers to extract style from and call them style layers denoted by $L_s$. In a similar manner, we choose one or several layers to extract content from, which we call content layers denoted by $L_c$. A convolutional layer $l$, with $N_l$ distinct filters has $N_l$ feature maps each of size $M_l$, where $M_l$ is the height times the width of the feature map. So, for a CNN model fed with an input $x$, the feature maps of a layer $l$ can be store in a matrix $F^l(x) \in R^{N_l \times M_l}$. The style of an image in this method, is represented as several Gram matrices, one for each style layer. The Gram matrix for each layer computes the correlation between different feature maps in that layer. For layer $l$ we have the Gram matrix $G^l(x) \in R^{N_l \times N_l}$, where $G_{ij}^l(x)$ is the inner product between the vectorised feature map $i$ and $j$ in layer $l$.

\begin{align}
    G_{ij}^l(x) = \sum_k^{} F_{ik}^l(x)F_{jk}^l(x)
\end{align}

We denote the Gram matrix for style layer $l$ of the CNN model fed with style image $x_s$ as $G^l(x_s)$ and the Gram matrix for style layer $l$ of the CNN model fed with the image generated as $G^l(x)$. The style loss is defined as the following.
\begin{align}
    &E_s^l(x) = \sum_{i, j}^{} (G_{ij}^l(x_s) - G_{ij}^l(x))^2\\
    &\Lagr_{\textit{style}}(x) = \sum_{l \in L_s}^{} E_s^l(x)
\end{align}

In a similar manner, the content loss is defined as the following.

\begin{align}
    &E_c^l(x) = \sum_{i, j}^{} (F_{i, j}^l(x_c) - F_{i, j}^l(x)) ^ 2\\
    &\Lagr_{\textit{content}}(x) = \sum_{l \in L_c}^{} E_c^l(x)
\end{align}

Where $F_{i,j}^l(x_c)$ is the feature maps of the CNN model fed with the content image and $F_{i,j}^l(x)$ is the feature maps of the CNN model fed with the generated image. 
The final loss is defined below.

\begin{align}
    \Lagr(x) = \Lagr_{\textit{style}}(x) + \lambda \Lagr_{\textit{content}}(x)
\end{align}

%%%%  Test Input Quality Metrics Math...

%%  Geometric Diversity...

Given $n$ test data, each producing $m$-dimensional feature vectors, we concatenate all the feature vectors into the matrix $V \in R^{n*m}$. The geometric diversity would be the following.\footnote{Note that since here we need to compute the determinant of a large matrix, the process would be numerically unstable. To overcome this phenomenon, we normalize the matrix $V$ and compute the logarithm of the determinant.}

\begin{align}
    G = det (V V^T)
\end{align}


%% STD...
Following the notation used for the geometric diversity, we have

\begin{align}
    \text{STD} = \left|\left|\left(\sqrt{\sum_{i=1}^{n}\frac{V_{i, j} - \mu_{j}}{n-1}}, 1 \leq j \leq m \right)\right|\right|
\end{align}

Where $\mu_j$ is the estimated mean of each component of feature vectors.


==> Sections/rq6_flaky.tex <==
\textbf{RQ6.} In this research question, we investigate if our current number of simulations are sufficient for a robust conclusion. Although we have conducted $100$ simulations for each ADS-DNN-Translator pair, as in Table \ref{fig:rq5_online}, we need to investigate the possibility of getting a significantly different result if we had conducted more experiments. We develop a statistical framework to analyze the robustness of our current results derived from simulations.

For offline testing, it is relatively easier, compared to online testing, to scale the testing as there are a handful of ways to increase test inputs. For example, one could easily use relevant image transformations to preserve label and generate more images to conduct offline testing on. In this manner, offline testing is easier to scale than online testing. However, in online testing, since we're using simulator which is cost-effective and time consuming, it is not generally cost and time-efficient to conduct more experiments. So, there is an urgent need to statistically and theoretically investigate whether we need more simulations or not to make a valid and reliable conclusion.

For every scenario $i$, we denote the fitness function when the translator is used as $F_{c,i}$ and the fitness function when no translator is used as $F_{r,i}$. As both $F_{c,i}$ and $F_{r,i}$ are calculated using averaging over thousands of time steps in a simulation, due to the central limit theorem, it's safe to assume they have Normal distributions. The difference between these two fitnesses is defined as $e_i = F_{c,i} - F_{r,i}$ which is also a Normal random variable. Since each scenario has its own simulation which is completely isolated from other scenarios and simulations, we can safely assume that all $e_i$s are independent and identically distributed (IID) and have Normal distribution. Let's assume that the true difference between the fitness function with and without corrector is a constant E which is unknown to us. Therefore, for each $e_i$ we have
\begin{align}
    e_i = E + n_i
\end{align}

In this formulation, $n_i$ is the noisy and flakiness effects causing the observed $e_i$ to be different from $E$. Due to independence of simulations and scenarios, we can safely assume $n_i$s to be independent and identically distributed and be observations of the random variable $N$. With no loss of generality, $N$ can be considered to have zero mean. Otherwise, we can add its non-zero mean to $E$ and define new $N^\prime = N - \EX\{N\}$ to have zero mean. Additionally, we denote the variance of $N$ as $\sigma^2$. Also note that a positive E, means that the translator helps getting better results in comparison with a no-translator online testing framework.

To estimate $E$, we can use an average estimator defined by the following.

\begin{align}
    \hat{E} = \frac{1}{m} \sum_{i=1}^m e_i
\end{align}

where $m$ is the number of observations. Now, let's compute the mean value of $\hat{E}$.
\begin{align}
    \EX\{\hat{E}\} &= \frac{1}{m} \sum_{i=1}^m \EX\{e_i\}\\
    &= \frac{1}{m} m.E\\
    &= E
\end{align}
So, $\hat{E}$ is an unbiased estimator of $E$ which is a desirable property for an estimator \cite{??}.

The variance of $\hat{E}$, denoted by $\hat{\sigma}^2$, is computed as the following.

\begin{align}
    \hat{\sigma}^2 &= \frac{1}{m^2} \sum_{i=1}^m \sigma^2\\
    &= \frac{1}{m} \sigma^2 \label{eqn:var}
\end{align}

Equation \ref{eqn:var} tells us that in order to reduce the uncertainty about the true value of $E$, we need to increase the number of observations (simulations).

Since each $e_i$ has a Normal distribution, $\hat{E}$, which is a linear combination of all $e_i$'s, is also a Normal random variable. So, we have $\hat{E} \sim \mathcal{N}(E, \frac{\sigma^2}{m})$.

Due to Normality of $\hat{E}$, we have the following inequality \cite{??}.

\begin{align}
    p\{E - 3\hat{\sigma} \leq \hat{E} \leq E + 3\hat{\sigma}\} \approx 0.997
\end{align}

So, for each ADSDNN-translator pair, we have an estimator $\hat{E}$, for which we have a lowerbound and an upperbound for its $99.7\%$ confidence interval. Table \ref{tab:rq6_bounds} shows the upperbound and lowerbound for each pair. A positive lower bound and upper bound for an ADSDNN-translator pair indicates that with a high confidence of $99.7$\%, using a translator is better than not using it for that ADS-DNN. However, we cannot infer that using translator is improving the testing if the lower bound is negative and the upper bound is positive. We could have such a conclusion only if both the lower bound and the upper bound are negative. Therefore, we can conclude that for example, for the Autumn ADS-DNN, all translators of Table \ref{tab:translators}, improve the online testing with an almost certain confidence of $99.7$\%. We can also conclude that for all ADS-DNNs of Table \ref{tab:adsdnns} except Dave2, SAEVAE can improve the online testing with a confidence of $99.7\%$.

\begin{table}[t]
    \centering
    \input{tables/bounds}
    \caption{Lower bounds and Upper bounds for $99.7\%$ confidence intervals for estimation of E for pairs of translators and ADSDNNs}
    \label{tab:rq6_bounds}
\end{table}

As we are interested in comparing different translator models, let's define the aforementioned $\hat{E}$ estimators for an ADS DNN using translators A and B as $\hat{E}_A$ and $\hat{E}_B$ respectively. We say that translator A is better than translator B if $\hat{E}_A > \hat{E}_B$. We define $D_{A,B} = \hat{E}_A - \hat{E}_B$. So, translator A is better than translator B if $D_{A,B} > 0$. A useful metric for comparing translators A and B, considering flakiness, would be the probability of $D_{A,B}$ being positive. In other words, we are interested in finding $p\{D_{A,B} > 0\}$. Since $D_{A,B}$ is defined as the sum (subtraction) of two Normal random variables, it has a Normal distribution. So, we have

\begin{align}
    D_{A,B} \sim \mathcal{N}(\hat{\mu}_{A,B}, \hat{\sigma}_{A,B}^2)
\end{align}

where $\hat{\mu}_{A,B} = \hat{E}_A - \hat{E}_B$ and $\hat{\sigma}_{A,B}^2 = \hat{\sigma}_A^2 + \hat{\sigma}_B^2$. 
Since $D_{A,B}$ is Normal random variable, we have

\begin{align}
    p\{D_{A,B} > 0 \} &= 1 - F(0) \\
    &= \frac{1}{2} [1 - \text{erf}(- \frac{\hat{\mu}_{A,B}}{\hat{\sigma}_{A,B} \sqrt{2}})]
\end{align}

Table \ref{tab:rq6_p} shows the probability of SAEVAE being better than cycleG and styleT for each ADS DNN.

\begin{table}[t]
    \centering
    \input{tables/pd}
    \caption{Probability of SAEVAE being better than other translators for each ADS DNN}
    \label{tab:rq6_p}
\end{table}




\begin{framed}
The answer to RQ6 is that in 5 out of 8 different comparisons of SAEVAE with other translators, across different ADS-DNNs, SAEVAE is doing better with probability of almost $1$. In 2 other cases, SAEVAE is better with a probability of at least 0.96. 
\end{framed}


==> headerpackages.tex <==
\usepackage{amsfonts}
\usepackage{ltl}

\usepackage{stmaryrd}
\usepackage{amsthm}
%\usepackage[utf8]{inputenc}
\usepackage{xcolor}
\usepackage[english]{babel} 
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{gensymb}
\usepackage{tikz}
\usepackage[inline]{enumitem}
\usepackage{numprint}
\usepackage{mathtools}
\usepackage[switch]{lineno}
\usepackage{gensymb}
\usepackage{amsmath}
\usepackage{fancybox}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage[xcolor=orange]{changes}
\usepackage{xcolor}
\usepackage[most]{tcolorbox}
\usepackage{fancybox}
\usepackage{pifont}% http://ctan.org/pkg/pifont

\newtcolorbox{mybox}[2][]{%  attach boxed title to top center
               %= {yshift=-8pt},
  colback      = gray!5!white,
  colframe     = gray!75!black,
  fonttitle    = \bfseries,
  colbacktitle = gray!85!black,
  left=0pt,
right=0pt,
top=0pt,
bottom=0pt,
%  title        = #2,#1,
 % enhanced,
}




\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}

%\newcommand\goal[1]{
%\noindent 
%\fcolorbox{black}{lightgray}{\noindent 
% \parbox{\columnwidth}{\noindent  #1}}\\
%}

\newcommand\objective[1]{
\vspace{0.1cm}
\noindent \fcolorbox{lightgray!40!black}{lightgray}{\parbox{0.98\columnwidth}{\noindent 
#1}}\vspace{0.1cm}\\
}


\definecolor{lightyellow}{rgb}{1.0, 1.0, 0.88}
\newcommand\defbox[1]{
\vspace{0.1cm}
\noindent \fcolorbox{lightyellow!40!black}{lightyellow}{\parbox{0.98\columnwidth}{\noindent 
#1}}\vspace{0.1cm}\\
}


\newcommand\resq[1]{
\noindent 
\fcolorbox{green!40!black}{green!5}{\noindent 
 \parbox{0.98\columnwidth}{\noindent  #1}}\\
}

\newcommand\hypothesis[1]{
\noindent 
\fcolorbox{yellow!40!black}{yellow!5}{\noindent 
 \parbox{0.98\columnwidth}{\noindent  #1}}\\
}


 \newcommand{\assumption}[2]{
\vspace{0.19cm} 
 \noindent \fcolorbox{black}{lightgray}{\parbox{0.98\columnwidth}{\noindent 
\textbf{\textsc{A#1.}} #2}}
\vspace{0.01cm}\\
} 
 
 
%  \newcommand{\assumption}[1]{\textbf{\textsc{A#1.}}} 




\definecolor{myBlue}{RGB}{0,133,255}%{HTML}{0085ff}
\definecolor{myGreen}{RGB}{0,115,0}

\newcommand\phase[1]{\tikz[baseline=(X.base)]\node [draw=myBlue,fill=myBlue,thick,rectangle,inner sep=2pt, rounded corners=2pt](X){\color{white}\textbf{#1}};}
\newcommand\phasenew[1]{\tikz[baseline=(X.base)]\node [draw=myGreen,fill=myGreen,thick,rectangle,inner sep=2pt, rounded corners=2pt](X){\color{white}\textbf{#1}};}


\newcommand\universeofInputs{\ensuremath{I}}
\newcommand\universeofOutputs{\ensuremath{O}}
\newcommand\universeofVariables{\ensuremath{V}}
\newcommand\interpretation[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand\specificationuniverse{S}
\newcommand\specification{s}
\newcommand\expectedoutputs{\ensuremath{E_o}}
\newcommand\timedomain{\ensuremath{\mathbb{T}}}
\newcommand\real{\ensuremath{\mathbb{R}}}
\newcommand\integer{\ensuremath{\mathbb{Z}}}
\newcommand\SFFOformula{\ensuremath{\varphi}}

\newcommand\formula{\ensuremath{\varphi}}
\newcommand\testcase{\ensuremath{\langle \timeinterval, \interpretation{\inputs}, \system \rangle}}


\newcommand\tollerableviolation{\ensuremath{\iota}}
\newcommand\noisevalues{\ensuremath{N}}
\newcommand\possibletestcase{\ensuremath{\langle \timedomain, \uncertainsystem,  \interpretation{\inputs}, \interpretation{\noises},   \interpretation{\parameters} \rangle}}



\newcommand\possibletestcaseprime{\ensuremath{\langle \timeinterval, \interpretation{\variables}, \interpretation{\inputsignals}, \noisevalues^\prime,  \system, \paramenters^\prime \rangle}}

\newcommand\partialsimulation{\ensuremath{F_o^\prime=H^\prime(t, \uncertainsystem,C, \interpretation{R},  \interpretation{F_i(n)}, N )}}

\newcommand\testoracle{\ensuremath{\system_\formula}}



\newcommand\uncertainsystem{\ensuremath{M_p}}



% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


\definechangesauthor[name={Claudio Menghi},color=orange]{CM}
\definechangesauthor[name={Shiva Nejati},color=red]{SN}
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}

\newboolean{showcomments}
\setboolean{showcomments}{true} % toggle to show or hide comments
\ifthenelse{\boolean{showcomments}}
{\newcommand{\nb}[2]{
  \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize#1}
  {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
 }
 \newcommand{\version}{\emph{\scriptsize$-$working$-$}}
}
{\newcommand{\nb}[2]{}
 \newcommand{\version}{}
}

\newcommand\claudio[1]{\nb{Claudio}{#1}}
\newcommand\shiva[1]{\nb{Shiva}{#1}}


 \newcommand{\goal}[1]{\textbf{\textsc{O#1}}} 

 
 \newcommand{\addedCM}[1]{\added[id=CM]{#1}}
\newcommand{\deletedCM}[1]{\deleted[id=CM]{#1}}
\newcommand{\replacedCM}[2]{\replaced[id=CM]{#2}{#1}}

\usepackage{makecell}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\partner}{LuxSpace}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}



\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{def}}}{=}}
\newcommand\variables{\ensuremath{R}}
\newcommand\signals{\ensuremath{F}}
\newcommand\inputsignals{\ensuremath{I}}

\newcommand\block{\ensuremath{B}}

\newcommand\inputsi{\ensuremath{F_i}}

\newcommand\timeinterval{\ensuremath{T}}
\newcommand\inputs{\ensuremath{I}}
\newcommand\inputsignal{\ensuremath{i}}
\newcommand\inputsuniverse{I}
\newcommand\noises{\ensuremath{\Delta}}
\newcommand\noise{\ensuremath{\delta}}

\newcommand\outputs{\ensuremath{O}}
\newcommand\outputsignal{\ensuremath{o}}

\newcommand{\powerset}{\raisebox{.15\baselineskip}{\Large\ensuremath{\wp}}}

\newcommand\risk{\emph{risk}}
\newcommand\diff{\emph{diff}}
\newcommand\ourlogic{RFOL}
\newcommand\casestudy{\textsf{SatEx}}
\newcommand\casestudyorbittime{two and a half hours}
\newcommand\casestudysimulationtime{YYYY minutes}
\newcommand\signaltrace{\ensuremath{w}}
\newcommand\variabletrace{\ensuremath{v}}
\newcommand\model{\ensuremath{\signaltrace}}
\newcommand\system{M}
\newcommand\parameters{\ensuremath{\Pi}}
\newcommand\parameter{\ensuremath{\pi}}

\newcommand\ourtool{\textttt{Sagacious}}


\newcommand\autopilot{Autopilot}
\makeatletter
\def\old@comma{,}
\catcode`\,=13
\def,{%
  \ifmmode%
    \old@comma\discretionary{}{}{}%
  \else%
    \old@comma%
  \fi%
}
\makeatother

\newcommand\term{\ensuremath{\theta}}
\newcommand\restrictedsffo{\ensuremath{RSFO}}


%\newcommand{\phase}[1]{%
%  \tikz[baseline=(text.base)]
%    {\node [draw,rounded corners] (text) {#1};}%
%}




%%%% Evaluation results

\npthousandsep{\,}






%\newcommand{\phase}[1]{%
%  \tikz[baseline=(text.base)]
%    {\node [draw,rounded corners] (text) {#1};}%
%}


\newcommand\numcasestudy{11}

\newtheorem{remark}{Remark}


%%%% Evaluation results
\newcommand\requirementNumber{90}
\newcommand\averageTimeOracleGeneration{1}
\newcommand\averageBlocksOracleGeneration{1}
\newcommand\averageConnectionsOracleGeneration{1}
\newcommand\averageSimulinkOracleGeneration{1}
\newcommand\averageSizeFormula{1}
\newcommand\percentagetimesaving{1\%}

\newcommand\newtext[1]{\color{blue} #1 \color{black}  }

\usepackage{algorithm}

\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{multirow}


==> letter/letter-revision.tex <==

\response{Thank you very much for the conditional accept decision and for reviewing a revised version of  our paper.\\[.5em]
The comments received from the reviewers have been extremely helpful in improving the paper, for which we are very grateful. We have completed \emph{all} the requested changes in the meta-review 
as detailed below:\\}

\noindent\textbf{Meta Review}

\rwcomment{comment1}{They provide evidence that the proposed approach outperforms the baseline in terms of OOB, not only OOB distance;}

\response{We now present the results for the number of out-of-bounds (OOBs) and the OOB distance values to better assess the translators' performance in ADS online testing. The new results, based on the number of OOBs, denoted by \#OOB, are consistent with the results and conclusions in our original submission. We have added the new \#OOB results to RQ3 and RQ6, which are the two research questions related to assessing online testing. Specifically, to present and discuss the new results, we have updated our paper as follows: (1)~We have introduced the \#OOB metric in Section~\ref{sec:evaluation}, lines 432-446. (2)~The RQ3 results in Tables~\ref{tab:rq4_online} and~\ref{tab:rq3_stattest} are now updated  with the \#OOB values. Further, the discussion of  RQ3 in Section~\ref{subsec:rq3} is updated and expanded based on these new results.  (3)~For RQ6, we have now added a new subtable, Table~\ref{tab:rq6(b)}, and a new table, Table~\ref{tab:rq6_pvals}, to present the new results related to \#OOB for this research question. Further, the discussion of RQ6 in Section~\ref{subsec:rq5} is updated and expanded.}

\rwcomment{comment2}{They provide a more detailed explanation regarding how simulated scenarios were built, the ground truth controller, and the default test input generation method;}

\response{We have now provided a detailed explanation of our method for generating simulated scenarios and test inputs for online testing in Section~\ref{subsec:setuponline}. Further, we now provide a detailed explanation related to the ground truths (i.e., labels) of the datasets used in our evaluation in Table~\ref{tab:train},  in Section~\ref{subsec:setupdnn} lines 498-506 and in Section~\ref{subsec:intval} lines 1136-1164. }

\rwcomment{comment3}{They discuss the threats to external validity that other more complex and comprehensive driving agents (e.g., Apollo and Autoware) and more advanced simulators like CARLA could have been considered in the evaluation.}

\response{We have now extended our threats to external validity section to mention the need for replicating our study with other ADS and simulators in the literature in Section~\ref{subsec:extval}.}

\response{In addition to addressing the changes requested in the meta-review, we have also provided further details regarding the training process for translators in Section~\ref{translator-setup}, Lines 552-565, as promised in our response to the reviews.  Finally, we have addressed all minor comments and typos raised by the reviewers.}



==> tables/bounds.tex <==
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{ADS DNN}                                          & \textbf{Translator} & \textbf{Lower Bound} & \textbf{Upper Bound} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Chauffeur}}} & SAEVAE             & 0.48007              & 1.066571             \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                    & cycleG           & -0.28041             & 0.245871             \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                    & styleT              & 0.069131             & 0.270766             \\ \hline
\multirow{3}{*}{\textbf{Autumn}}                          & SAEVAE             & 0.684273             & 1.212431             \\ \cline{2-4} 
                                                          & cycleG           & 0.084973             & 0.475477             \\ \cline{2-4} 
                                                          & styleT              & 0.01505              & 0.304811             \\ \hline
\multirow{3}{*}{\textbf{Epoch}}                           & SAEVAE             & 0.326692             & 0.54202              \\ \cline{2-4} 
                                                          & cycleG           & 0.195825             & 0.463386             \\ \cline{2-4} 
                                                          & styleT              & 0.09629              & 0.220892             \\ \hline
\multirow{3}{*}{\textbf{Dave2}}                           & SAEVAE             & -0.01147             & 0.062059             \\ \cline{2-4} 
                                                          & cycleG           & -0.16452             & 0.195402             \\ \cline{2-4} 
                                                          & styleT              & -0.1172              & 0.036793             \\ \hline
\end{tabular}

==> tables/pd.tex <==
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{ADS DNN}                                          & \textbf{Translator A} & \textbf{Translator B} & $p\{D_{A,B} > 0\}$ \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Chauffeur}}} & SAEVAE               & cycleG             & 1          \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                    & SAEVAE               & styleT                & 1          \\ \hline
\multirow{2}{*}{\textbf{Autumn}}                          & SAEVAE               & cycleG             & 1          \\ \cline{2-4} 
                                                          & SAEVAE               & styleT                & 1          \\ \hline
\multirow{2}{*}{\textbf{Epoch}}                           & SAEVAE               & cycleG             & 0.966      \\ \cline{2-4} 
                                                          & SAEVAE               & styleT                & 1          \\ \hline
\multirow{2}{*}{\textbf{Dave2}}                           & SAEVAE               & cycleG             & 0.564      \\ \cline{2-4} 
                                                          & SAEVAE               & styleT                & 0.989      \\ \hline
\end{tabular}

==> tables/tab_adsdnns.tex <==
\begin{table}[t]
\centering
\caption{ADS-DNNs}
\label{tab:adsdnns}
\scalebox{0.9}{
\begin{tabular}{|l|l|l|}
\hline
\textbf{ADS-DNN}   & \textbf{Source} & \textbf{Training process and Parameters} \\ \hline
\textbf{Autumn}    &  \cite{??}               &                                    \\ \cline{1-2}
\textbf{Chauffeur} &      \cite{??}           & All models are trained on a random $70$\% split                                 \\ \cline{1-2}
\textbf{Dave2}     &    \cite{??}             &  of $D_{real}$ with             50 Epochs, Batch Size = 128.                 \\ \cline{1-2}
\textbf{Epoch}     &    \cite{??}             &                           \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_ds.tex <==
\begin{table}[t]
\centering
\caption{Datasets}
\label{tab:datasets}
\scalebox{1}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Dataset}    & \textbf{Source} & \textbf{Size} & \textbf{Input Size} & \textbf{Output Range} \\ \hline
\textbf{$D_{real}$} & \cite{??}     & 3376          & (160, 320, 3)       & {[}-1, 1{]}           \\ \hline
\textbf{$D_{sim}$}  & \cite{??}     & 8563          & (160, 320, 3)       & {[}-1, 1{]}           \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq2_offline.tex <==
\begin{table}[t]
\centering
\caption{MAE results of ADS-DNNs for real-world ($D_{\mathit{real}}$) and simulator-generated  ($D_{\mathit{sim}}$) datasets}
\label{tab:rq2_offline}
\begin{tabular}{lrrr}
\toprule
{} &  $D_{\mathit{real}}$ &  $D_{\mathit{sim}}$ & $\Delta_{(\mathit{real}, \mathit{sim})}$  \\
\midrule
Dave2  &          0.38 &   0.50 & -0.12 \\
Chauffeur &          0.20 &   0.42 & -0.22 \\
Epoch     &          0.24 &   0.35& -0.11\\
Autumn &          0.14 &   0.85& -0.71\\
\bottomrule
\end{tabular}
\end{table}

==> tables/tab_rq2_raw.tex <==
\begin{table}[t]
\centering
\caption{Mean and standard deviation of Mean OOB of all scenarios for ADS-DNNs}
\label{tab:rq2_raw}
\begin{tabular}{lrrrr}
\toprule
{} &  Chauffeur &   Autumn &     Epoch &    Dave2 \\
\midrule
Mean &   1.156641 &  1.189536 &  1.163185 &  1.60760 \\
Std  &   0.795898 &  0.673823 &  0.615509 &  0.69899 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/tab_rq3_offline.tex <==
\begin{table}[t]
\centering
\caption{Average accuracy (MAE)  of ADS-DNNs on the  simulator generated dataset ($D_{\mathit{sim}}$) translated by SAEVAE, StyleTransfer and CycleGAN translators, respectively}
\label{tab:rq3_offline}
\scalebox{0.8}{
\begin{tabular}{lrrr}
\toprule
{} &  $\mathit{saevae(}D_{\mathit{sim}})$ &  $\mathit{styleT(}D_{\mathit{sim}})$ &  $\mathit{cycleG(}D_{\mathit{sim}})$ \\
\midrule
Dave2 &            0.484  &  0.484 &  0.484\\
Chauffeur &            0.352  &  0.394 &  0.469 \\
Epoch     &           0.254  &  0.321 & 0.406 \\
Autumn &             0.367  &  0.803  & 0.517 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/tab_rq4_blackbox_old.tex <==
\begin{table}[t]
\centering
\caption{Percentage differences in Black-box test data quality metrics, Geometric Diversity (GD), and Standard Deviation (STD), for synthetic dataset with and without translators, relative to $\text{D}_{\text{sim}}$.}
\label{tab:rq4_blackbox}
\scalebox{0.8}{
\begin{tabular}{|l|l|c|c|}
\hline
\multicolumn{1}{|c|}{Task} & \multicolumn{1}{c|}{Dataset} & GD & STD \\ \hline
\multirow{3}{*}{Lane Keeping} & SAEVAE  & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 33.03\% \\ \cline{2-4}
                              & cycleG  & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 24.32\% \\ \cline{2-4}
                              & styleT  & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 11.07\% \\ \hline
\multirow{3}{*}{Object Detection} & SAEVAE & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 4.04\% \\ \cline{2-4}
                                   & cycleG & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 16.11\% \\ \cline{2-4}
                                   & styleT & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 3.36\% \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq4_nc.tex <==
\begin{table}[t]
\centering
\caption{Percentage differences in Neuron Coverage for each dataset relative to $\text{D}_{\text{sim}}$}
\label{tab:rq4_nc_relative}
\scalebox{1.2}{
\begin{tabular}{|l|C|C|C|C|}
\hline
Dataset & Autumn & Chauffeur & Dave2 & Epoch \\ \hline
SAEVAE  & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 2\% & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 3\% \\ \hline
cycleG  & \cellcolor{green!25}$\approx$ & \cellcolor{green!25}↑ 5\% & \cellcolor{green!25}$\approx$ & \cellcolor{green!25}↑ 3\% \\ \hline
styleT  & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 3\% & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 3\% \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq4_nc_old.tex <==
\begin{table}[t]
\centering
\caption{Neuron Coverage}
\label{tab:rq4_nc}
\scalebox{1.2}{
\begin{tabular}{|l|l|l|l|l|}
\hline
Dataset & Autumn & Chauffeur & Dave2 & Epoch \\ \hline
DS\_sim & 0.9    & 0.47      & 0     & 0.51  \\ \hline
SAEVAE  & 0.9    & 0.45      & 0     & 0.48  \\ \hline
cycleG  & 0.9    & 0.52      & 0.4   & 0.54  \\ \hline
styleT  & 0.9    & 0.44      & 0     & 0.48  \\ \hline
\end{tabular}
}
\end{table}


==> tables/tab_rq4_onlinestat.tex <==
\begin{table}[t]
\centering
\caption{\#OOB for $100$ online testing scenarios applied to four 
lane-keeping ADS-DNNs with and without translators}
\label{tab:rq4_online_stat}
\scalebox{0.55}{
\begin{tabular}{|l|cc|cc|cc|}
\hline
\multirow{3}{*}{\textbf{ADS DNN}} & \multicolumn{2}{c|}{\textbf{SAEVAE vs No Translator}}                              & \multicolumn{2}{c|}{\textbf{SAEVAE vs cycleG}}                                  & \multicolumn{2}{c|}{\textbf{SAEVAE vs styleT}}                                  \\ \cline{2-7} 
                                  & \multicolumn{2}{c|}{\textbf{\#OOB}}                                              & \multicolumn{2}{c|}{\textbf{\#OOB}}                                           & \multicolumn{2}{c|}{\textbf{\#OOB}}                                           \\ \cline{2-7} 
                                  & \multicolumn{1}{c|}{\textbf{A12}} & \textbf{p-value} & \multicolumn{1}{c|}{\textbf{A12}} & \textbf{p-value} & \multicolumn{1}{c|}{\textbf{A12}} & \textbf{p-value} \\ \hline
\textbf{Autumn}                   & \multicolumn{1}{c|}{0.46}         & 0.00             & \multicolumn{1}{c|}{0.46}         & 0.94             & \multicolumn{1}{c|}{0.42}         & 0                \\ \hline
\textbf{Chauffeur}                & \multicolumn{1}{c|}{0.43}         & 0.00             & \multicolumn{1}{c|}{0.41}         & 0.00             & \multicolumn{1}{c|}{0.42}         & 0                \\ \hline
\textbf{Dave2}                    & \multicolumn{1}{c|}{0.45}         & 0.00             & \multicolumn{1}{c|}{0.31}         & 0.00             & \multicolumn{1}{c|}{0.36}         & 0                \\ \hline
\textbf{Epoch}                    & \multicolumn{1}{c|}{0.51}         & 0.83             & \multicolumn{1}{c|}{0.57}         & 0.14             & \multicolumn{1}{c|}{0.53}         & 0.3              \\ \hline
\end{tabular}
}
\end{table}


==> tables/tab_rq4_sa.tex <==
\begin{table}[t]
\centering
\caption{Percentage difference of surprising examples based on surprise adequacy metric, relative to $\text{D}_{\text{sim}}$}
\label{tab:rq4_sa_relative_arrows_colors}
\scalebox{1.2}{
\begin{tabular}{|l|C|C|C|C|}
\hline
Dataset & Autumn & Chauffeur & Dave2 & Epoch \\ \hline
SAEVAE  & \cellcolor{yellow!25}↓ 3\% & \cellcolor{green!25}$\approx$ & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 39\% \\ \hline
cycleG  & \cellcolor{green!25}↑ 1\% & \cellcolor{green!25}$\approx$ & \cellcolor{yellow!25}↓ 96\% & \cellcolor{yellow!25}↓ 69\% \\ \hline
styleT  & \cellcolor{yellow!25}↓ 2\% & \cellcolor{green!25}$\approx$ & \cellcolor{green!25}$\approx$ & \cellcolor{green!25}$\approx$ \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq4_sa_old.tex <==
\begin{table}[t]
\centering
\caption{Percentage of surprising examples based on surprise adequacy metric.}
\label{tab:rq4_sa}
\scalebox{1.2}{
\begin{tabular}{|l|l|l|l|l|}
\hline
Dataset & Autumn & Chauffeur & Dave2 & Epoch \\ \hline
DS\_sim & 0.03   & 1         & 1     & 1     \\ \hline
SAEVAE  & 0      & 1         & 1     & 0.61  \\ \hline
cycleG  & 0.04   & 1         & 0.04  & 0.31  \\ \hline
styleT  & 0.01   & 1         & 1     & 1     \\ \hline
\end{tabular}
}
\end{table}


==> tables/tab_rq5_corr_detailed.tex <==
\begin{table}[t]
\centering
\caption{Mean of Pearson and Spearman correlation between offline testing (MAE) and online testing (OOB) across test scenarios}
\label{tab:rq5_corr}
\scalebox{0.6}{
\begin{tabular}{|l|l|lll|lll|}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{ADS-DNN} & \multicolumn{3}{c|}{Pearson}                                                    & \multicolumn{3}{c|}{Spearman}                                                   \\ \cline{3-8} 
                        &                          & \multicolumn{1}{l|}{Translator} & \multicolumn{1}{l|}{w/o Translator} & diff    & \multicolumn{1}{l|}{Translator} & \multicolumn{1}{l|}{w/o Translator} & diff    \\ \hline
\multirow{5}{*}{SAEVAE} & Autumn                   & \multicolumn{1}{l|}{-0.6}       & \multicolumn{1}{l|}{0.65}           & -0.05   & \multicolumn{1}{l|}{-0.68}      & \multicolumn{1}{l|}{0.6}            & 0.08    \\ \cline{2-8} 
                        & Chauffeur                & \multicolumn{1}{l|}{-0.72}      & \multicolumn{1}{l|}{0.39}           & 0.33    & \multicolumn{1}{l|}{-0.73}      & \multicolumn{1}{l|}{0.51}           & 0.22    \\ \cline{2-8} 
                        & Dave2                    & \multicolumn{1}{l|}{0.12}       & \multicolumn{1}{l|}{0.11}           & 0.01    & \multicolumn{1}{l|}{0.04}       & \multicolumn{1}{l|}{0.01}           & 0.03    \\ \cline{2-8} 
                        & Epoch                    & \multicolumn{1}{l|}{-0.49}      & \multicolumn{1}{l|}{0.52}           & -0.03   & \multicolumn{1}{l|}{-0.37}      & \multicolumn{1}{l|}{0.71}           & -0.34   \\ \cline{2-8} 
                        & Mean                     & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}               & \cellcolor{green!25}0.065   & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}               & \cellcolor{yellow!25}-0.0025 \\ \hline
\multirow{5}{*}{cycleG} & Autumn                   & \multicolumn{1}{l|}{0.5}        & \multicolumn{1}{l|}{0.65}           & -0.15   & \multicolumn{1}{l|}{0.45}       & \multicolumn{1}{l|}{0.6}            & -0.15   \\ \cline{2-8} 
                        & Chauffeur                & \multicolumn{1}{l|}{0.77}       & \multicolumn{1}{l|}{0.39}           & 0.38    & \multicolumn{1}{l|}{0.74}       & \multicolumn{1}{l|}{0.51}           & 0.23    \\ \cline{2-8} 
                        & Dave2                    & \multicolumn{1}{l|}{-0.53}      & \multicolumn{1}{l|}{0.11}           & 0.42    & \multicolumn{1}{l|}{-0.55}      & \multicolumn{1}{l|}{0.01}           & 0.54    \\ \cline{2-8} 
                        & Epoch                    & \multicolumn{1}{l|}{0.32}       & \multicolumn{1}{l|}{0.52}           & -0.2    & \multicolumn{1}{l|}{0.41}       & \multicolumn{1}{l|}{0.71}           & -0.3    \\ \cline{2-8} 
                        & Mean                     & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}               & \cellcolor{green!25}0.1125  & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}               & \cellcolor{green!25}0.08    \\ \hline
\multirow{5}{*}{Style}  & Autumn                   & \multicolumn{1}{l|}{0.69}       & \multicolumn{1}{l|}{0.65}           & 0.04    & \multicolumn{1}{l|}{0.71}       & \multicolumn{1}{l|}{0.6}            & 0.11    \\ \cline{2-8} 
                        & Chauffeur                & \multicolumn{1}{l|}{0.3}        & \multicolumn{1}{l|}{0.39}           & -0.09   & \multicolumn{1}{l|}{0.46}       & \multicolumn{1}{l|}{0.51}           & -0.05   \\ \cline{2-8} 
                        & Dave2                    & \multicolumn{1}{l|}{0.01}       & \multicolumn{1}{l|}{0.11}           & -0.1    & \multicolumn{1}{l|}{-0.08}      & \multicolumn{1}{l|}{0.01}           & 0.07    \\ \cline{2-8} 
                        & Epoch                    & \multicolumn{1}{l|}{0.52}       & \multicolumn{1}{l|}{0.52}           & 0       & \multicolumn{1}{l|}{0.68}       & \multicolumn{1}{l|}{0.71}           & -0.03   \\ \cline{2-8} 
                        & Mean                     & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}               & \cellcolor{yellow!25}-0.0375 & \multicolumn{1}{l|}{}           & \multicolumn{1}{l|}{}               & \cellcolor{green!25}0.025   \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq5_corr_old.tex <==
\begin{table}[t]
\centering
\caption{Correlation difference between using translator and not using translator. Each correlation is calculated between offline testing (MAE) and online testing (OOB) across test scenarios}
\label{tab:rq5_corr}
\scalebox{0.7}{
\begin{tabular}{|l|l|ll|}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{ADS-DNN} & \multicolumn{2}{l|}{Correlation Difference} \\ \cline{3-4} 
                        &                          & \multicolumn{1}{l|}{Pearson}   & Spearman   \\ \hline
\multirow{4}{*}{SAEVAE} & Autumn                   & \multicolumn{1}{l|}{-0.05}     & 0.08       \\ \cline{2-4} 
                        & Chauffeur                & \multicolumn{1}{l|}{0.33}      & 0.22       \\ \cline{2-4} 
                        & Dave2                    & \multicolumn{1}{l|}{0.01}      & 0.03       \\ \cline{2-4} 
                        & Epoch                    & \multicolumn{1}{l|}{-0.03}     & -0.34      \\ \hline
\multirow{4}{*}{cycleG} & Autumn                   & \multicolumn{1}{l|}{-0.15}     & -0.15      \\ \cline{2-4} 
                        & Chauffeur                & \multicolumn{1}{l|}{0.38}      & 0.23       \\ \cline{2-4} 
                        & Dave2                    & \multicolumn{1}{l|}{0.42}      & 0.54       \\ \cline{2-4} 
                        & Epoch                    & \multicolumn{1}{l|}{-0.2}      & -0.3       \\ \hline
\multirow{4}{*}{styleT} & Autumn                   & \multicolumn{1}{l|}{0.04}      & 0.11       \\ \cline{2-4} 
                        & Chauffeur                & \multicolumn{1}{l|}{-0.09}     & -0.05      \\ \cline{2-4} 
                        & Dave2                    & \multicolumn{1}{l|}{-0.1}      & 0.07       \\ \cline{2-4} 
                        & Epoch                    & \multicolumn{1}{l|}{0}         & -0.03      \\ \hline
\end{tabular}
}
\end{table}


==> tables/tab_rq5_ncsa_obj.tex <==
\begin{table}[t]
\centering
\caption{Percentage differences in Neuron Coverage (NC) and Surprise Adequacy (SA) relative to $\text{D}_{\text{sim}}$}
\label{tab:rq4_ncsa}
\scalebox{0.8}{
\begin{tabular}{|l|c|c|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{YOLO} \\ \cline{2-3} 
                         & NC          & SA            \\ \hline
SAEVAE                   & \cellcolor{green!25}↑ 2\% & \cellcolor{yellow!25}↓ 3\%  \\ \hline
cycleG                   & \cellcolor{yellow!25}↓ 9\% & \cellcolor{green!25}↑ 24\%  \\ \hline
styleT                   & \cellcolor{yellow!25}↓ 3\% & \cellcolor{green!25}↑ 4\%  \\ \hline

\end{tabular}
}
\end{table}

==> tables/tab_rq5_offlinetime.tex <==
\begin{table}[t]
\centering
\caption{Average inference time for each translator}
\label{tab:rq5_offlinetime}
\scalebox{1}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Translator} & SAEVAE & cycleG & styleT \\ \hline
\textbf{Time}       & 0.05s  & 0.30s     & 4.69s         \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq6_oob85.tex <==
\begin{table}[t]
\centering
\caption{The differences in average correlation between online and offline test results with translators compared to those without translators: Positive values indicate that translators improve the correlation, while negative values indicate that they decrease the correlation}
\label{tab:rq5_corr}
\scalebox{0.85}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Translator}              & \textbf{Correlation} & \textbf{Autumn} & \textbf{Chauffeur} & \textbf{Dave2} & \textbf{Epoch} \\ \hline
\multirow{2}{*}{\textbf{SAEVAE}} & Pearson              & 0.11            & 1.25               & -0.06          & 0.31           \\ \cline{2-6} 
                                 & Spearman             & 0.61            & 1.14               & -0.09          & 0.44           \\ \hline
\multirow{2}{*}{\textbf{cycleG}} & Pearson              & -0.64           & 0.56               & 0.59           & 0.04           \\ \cline{2-6} 
                                 & Spearman             & -0.18           & 0.29               & 0.63           & -0.06          \\ \hline
\multirow{2}{*}{\textbf{styleT}} & Pearson              & 0.08            & -0.25              & 0.01           & 0.09           \\ \cline{2-6} 
                                 & Spearman             & 0.50            & -0.27              & -0.07          & 0.15           \\ \hline
\end{tabular}
}
\end{table}

==> tables/tab_rq6_pvals.tex <==
\begin{table}[t]
\vspace*{.25cm}
\centering
\caption{The p-values for the Pearson and Spearman correlations computed between MAE and OOB, and between MAE and $\#$OOB for each ADS-DNN, calculated both without a translator and with each of the SAEVAE, cycleG, and styleT translators. All p-values are near zero, indicating high confidence in the correlations}
\label{tab:rq6_pvals}
\vspace*{-.2cm}
\scalebox{0.65}{
\begin{tabular}{|l|l|ll|ll|}
\hline
\multirow{2}{*}{\textbf{Translator}}     & \multirow{2}{*}{\textbf{ADS-DNN}} & \multicolumn{2}{l|}{\textbf{OOB distance}}                & \multicolumn{2}{l|}{\textbf{$\#$OOB}}                       \\ \cline{3-6} 
                                         &                                   & \multicolumn{1}{l|}{\textbf{Pearson}} & \textbf{Spearman} & \multicolumn{1}{l|}{\textbf{Pearson}} & \textbf{Spearman} \\ \hline
\multirow{4}{*}{\textbf{w/o translator}} & Autumn                            & \multicolumn{1}{l|}{$\sim$ 0}        & 0                 & \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Chauffeur                         & \multicolumn{1}{l|}{0}                & 0                 & \multicolumn{1}{l|}{$\sim$ 0}        & $\sim$ 0\\ \cline{2-6} 
                                         & Dave2                             & \multicolumn{1}{l|}{$\sim$ 0}         & 0                 & \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Epoch                             & \multicolumn{1}{l|}{$\sim$ 0}         & $\sim$ 0& \multicolumn{1}{l|}{0}                & 0                 \\ \hline
\multirow{4}{*}{\textbf{SAEVAE}}         & Autumn                            & \multicolumn{1}{l|}{$\sim$ 0}                 & $\sim$ 0& \multicolumn{1}{l|}{$\sim$ 0}         & $\sim$ 0\\ \cline{2-6} 
                                         & Chauffeur                         & \multicolumn{1}{l|}{$\sim$ 0}         & $\sim$ 0& \multicolumn{1}{l|}{$\sim$ 0}        & $\sim$ 0\\ \cline{2-6} 
                                         & Dave2                             & \multicolumn{1}{l|}{0}                & 0                 & \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Epoch                             & \multicolumn{1}{l|}{$\sim$ 0}         & $\sim$ 0& \multicolumn{1}{l|}{$\sim$ 0}        & $\sim$ 0\\ \hline
\multirow{4}{*}{\textbf{cycleG}}         & Autumn                            & \multicolumn{1}{l|}{0}                & $\sim$ 0& \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Chauffeur                         & \multicolumn{1}{l|}{0}                & 0                 & \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Dave2                             & \multicolumn{1}{l|}{$\sim$ 0}         & 0                 & \multicolumn{1}{l|}{$\sim$ 0}         & $\sim$ 0\\ \cline{2-6} 
                                         & Epoch                             & \multicolumn{1}{l|}{0}                & 0                 & \multicolumn{1}{l|}{0}                & 0                 \\ \hline
\multirow{4}{*}{\textbf{styleT}}& Autumn                            & \multicolumn{1}{l|}{$\sim$ 0}        & $\sim$ 0& \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Chauffeur                         & \multicolumn{1}{l|}{0}                & $\sim$ 0& \multicolumn{1}{l|}{0}                & $\sim$ 0\\ \cline{2-6} 
                                         & Dave2                             & \multicolumn{1}{l|}{0}                & 0                 & \multicolumn{1}{l|}{0}                & 0                 \\ \cline{2-6} 
                                         & Epoch                             & \multicolumn{1}{l|}{0}                & $\sim$ 0& \multicolumn{1}{l|}{0}                & 0                 \\ \hline
\end{tabular}
}
% \vspace*{0.1cm}
\end{table}

==> tables/tab_translators.tex <==
\begin{table}[t]
\centering
\caption{Translators. }
\label{tab:translators}
\scalebox{0.72}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Translator} & \textbf{Source} & \textbf{Source Domain} & \textbf{Target Domain} & \textbf{Training Parameters} \\ \hline
\textbf{SAEVAE}     &  \cite{??}               & $D_{sim}$              & $D_{real}$             &         $\alpha = 1$                     \\ \hline
\textbf{CycleG}     &    \cite{??}             & $D_{sim}$              & $D_{real}$             & $\lambda = 0.9$         \\ \hline
\textbf{StyleT}     &   \cite{??}           & $D_{sim}$              & Random x  $ \in D_{real}$             &   $\beta = 100$        \\ \hline
\end{tabular}
}
\end{table}

==> todo.tex <==
Aug 9:

References added --> MH (Done)

Spacing

Proofreading

Line numbers --> MH  (Done)

Fig 5 --> D\_real should be D\_real, test  --> MH (Done)

References  checked --> MH (Done)
